Arm DynamIQ Shared Unit and Real-Time: An Empirical Evaluation

The increasing complexity of embedded hardware platforms poses significant challenges for real-time workloads. Architectural features such as Intel RDT, Arm QoS, and Arm MPAM are either unavailable on commercial embedded platforms or designed primarily for server environments optimized for average-case performance and might fail to deliver the expected real-time guarantees. Arm DynamIQ Shared Unit (DSU) includes isolation features-among others, hardware per-way cache partitioning-that can improve the real-time guarantees of complex embedded multicore systems and facilitate real-time analysis. However, the DSU also targets average cases, and its real-time capabilities have not yet been evaluated. This paper presents the first comprehensive analysis of three real-world deployments of the Arm DSU on Rockchip RK3568, Rockchip RK3588, and NVIDIA Orin platforms. We integrate support for the DSU at the operating system and hypervisor level and conduct a large-scale evaluation using both synthetic and real-world benchmarks with varying types and intensities of interference. Our results make extensive use of performance counters and indicate that, although effective, the quality of partitioning and isolation provided by the DSU depends on the type and the intensity of the interfering workloads. In addition, we uncover and analyze in detail the correlation between benchmarks and different types and intensities of interference.

==> Makefile <==
PROJNAME=paper
OUTDIR=out

TEXINC := \
	0-notation.tex \
	0-abstract.tex \
	1-introduction.tex \
	2-related.tex \
	5-implementation.tex \
	6-eval.tex \
	7-conclusion.tex

.PHONY: all clean distclean .FORCE

all : $(PROJNAME).pdf

pdf : $(PROJNAME).pdf

$(PROJNAME).pdf: $(PROJNAME).tex $(TEXINC) $(PROJNAME).bib
	latexmk -pdf -bibtex -output-directory=$(OUTDIR) -use-make $<
	@echo "=============================================="
	@grep Warning $(OUTDIR)/paper.log || echo "No warnings."

distclean:
	rm -rf $(OUTDIR)
	rm -f *~ *.aux *.backup *.blg *.log *.out *.lof *.bbl *.bak *.vtc *.fdb_latexmk

clean:
	latexmk -output-directory=$(OUTDIR) -c


==> figures.tex <==
% \newcommand{\figureA}{
%     \begin{figure}[h!]
%         \centering
%         \includegraphics[width=\columnwidth]{figures/prefetch_plru.eps}
%         \caption{Plot for Synthetic Benchmark}
%         \label{fig:prefetch-plru}
%     \end{figure}
%     }

% \newcommand{\figureB}{
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/sythetic_plot.eps}
%     \caption{Plot for Synthetic Benchmark}
%     \label{fig:synthetic-plot}
% \end{figure}
% }

% \newcommand{\figureC}{
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/no_partition_perf.eps}
%     \caption{Performance Counters in No Partitioning}
%     \label{fig:no-partition-perf}
% \end{figure}
% }

% \newcommand{\figureD}{
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/percent_change_no_partition_modify_vga.eps}
%     \caption{No Partitioning - Change in Execution Time}
%     \label{fig:percent-no-partition-modify-vga}
% \end{figure}
% }

% \newcommand{\figureE}{
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/rk3568_set__percent_mser_modify_vga.eps}
%     \caption{Set Partitioning in RK3568 modify vs mser/vga}
%     \label{fig:rk3568-set-mser-modify-vga}
% \end{figure}
% }

% \newcommand{\figureF}{
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/rk3568_way__percent_mser_modify_vga.eps}
%     \caption{Way Partitioning in RK3568 modify vs mser/vga}
%     \label{fig:rk3568-way-mser-modify-vga}
% \end{figure}
% }

% \newcommand{\figureG}{
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/rk3568_way__percent_disparity_modify_vga.eps}
%     \caption{FIXME: Way Partitioning in RK3568 modify vs disparity/vga}
%     \label{fig:rk3568-way-disparity-modify-vga}
% \end{figure}
% }

% \newcommand{\figureH}{
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/rk3588_set__percent_mser_prefetch_l3_vga.eps}
%     \caption{Set Partitioning in RK3588 prefetch_l3 vs mser/vga}
%     \label{fig:rk3588-set-mser-prefetch-vga}
% \end{figure}
% }

% \newcommand{\figureI}{
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/rk3588_way__percent_mser_prefetch_l3_vga.eps}
%     \caption{Way Partitioning in RK3588 prefetch_l3 vs mser/vga}
%     \label{fig:rk3588-way-mser-prefetch-vga}
% \end{figure}
% }

% \newcommand{\figureJ}{
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/rk3588_way__percent_mser_modify_vga.eps}
%     \caption{FIXME: Way Partitioning in RK3588 prefetch_l3 vs mser/vga}
%     \label{fig:rk3588-way-mser-modify-vga}
% \end{figure}
% }

% \newcommand{\figureK}{
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/44_45_mser_modify.eps}
%     \caption{Performance Counters for modify vs mser/vga in RK3588}
%     \label{fig:44-45-mser-modify}
% \end{figure}
% }

% \newcommand{\figureL}{
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/64_modify_rk3568.eps}
%     \caption{Performance Counter for modify interference-bench in RK3568}
%     \label{fig:64-modify-rk3568}
% \end{figure}
% }

% \newcommand{\figureM}{
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/rk3588_set__percent_disparity_write_cif.eps}
%     \caption{Set Partitioning on RK3588 for write interference with the disparity/cif benchmark}
%     \label{fig:rk3588-set-disparity-cif}
% \end{figure}
% }

% \newcommand{\figureN}{
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/zcu102_set__percent_disparity_write_cif.png}
%     \caption{Set Partitioning on ZCU102 for write interference with the disparity/cif benchmark}
%     \label{fig:zcu102-set-disparity-cif}
% \end{figure}
% }

